Low-Cost On-device Partial Domain Adaptation (LoCO-PDA): Enabling efficient CNN retraining on edge devices

With the increased deployment of Convolutional Neural Networks (CNNs) on edge devices, the uncertainty of the observed data distribution upon deployment has led researchers to to utilise large and extensive datasets such as ILSVRC'12 to train CNNs. Consequently, it is likely that the observed data distribution upon deployment is a subset of the training data distribution. In such cases, not adapting a network to the observed data distribution can cause performance degradation due to negative transfer and alleviating this is the focus of Partial Domain Adaptation (PDA). Current works targeting PDA do not focus on performing the domain adaptation on an edge device, adapting to a changing target distribution or reducing the cost of deploying the adapted network. This work proposes a novel PDA methodology that targets all of these directions and opens avenues for on-device PDA. LoCO-PDA adapts a deployed network to the observed data distribution by enabling it to be retrained on an edge device. Across subsets of the ILSVRC12 dataset, LoCO-PDA improves classification accuracy by 3.04pp on average while achieving up to 15.1x reduction in retraining memory consumption and 2.07x improvement in inference latency on the NVIDIA Jetson TX2. The work is open-sourced at \emph{link removed for anonymity}.

==> extra.tex <==
\section{Further Experiments}
    \label{sec:further_experiments}
    This section discusses additional experiments performed to identify the limits of LoCO-PDA.
    
    \subsection{Other network architectures}
        \label{sec:fe_other_network_architectures}
        \input{tables_tex/further_experiments/mobilenet_v2_50_acc.tex}
        \subsubsection{MobileNetV2 \cite{mobilenetv2_Sandler2018}}
            The results from Sec.\ref{sec:evaluation} demonstrate that LoCO-PDA generalises well
            across different pruning strategies (TFO, OFA) for the same backbone network
            (ResNet50).
            This section evaluates LoCO-PDA's generalisability to other networks by evaluating it
            on MobileNetV2.
            Table.\ref{tab:mobv2_acc_comparison} displays the accuracy regained by performing
            on-device memory limited, classifier-only training and LoCO-PDA on the four autonomous
            driving $\mathcal{D}'$. 
            $\mathcal{M}^0_{TFO}$ is an unpruned MobileNetV2 with 312.3 MFLOPs of inference cost
            and 14.09 MB of model memory.
            $\mathcal{M}^{50}_{TFO}$ is a 50\% TFO pruned MobileNetV2 network with 166.6 MFLOPs of
            inference cost and 7.06 MB of model memory.
            
            Across all $\mathcal{D}'$, LoCO-PDA performs 0.88pp better than memory limited
            classifier-only retraining.
            However, although the image based retraining methodology degrades accuracy by 9.01pp in
            the label uncertain setting compared to label certain setting, LoCO-PDA also degrades
            accuracy by 2.45pp. 
            This could be due to the lower accuracy of the unpruned MobileNetV2 compared to the
            networks in Sec.\ref{sec:evaluation}, thus demonstrating the sensitivity of LoCO-PDA to
            an overly noisy estimation of $\mathcal{D}'$. 

        \subsubsection{VGG11 \cite{vgg_Simonyan_15}}
            All the networks evaluated thus far and all modern CNN architectures have linear
            classifiers while AlexNet \cite{alexnet} and VGG11 \cite{vgg_Simonyan_15} have
            non-linear classifiers. %comprised of 3 fully connected layers with ReLU
            non-linearities inbetween.
            % This pattern implies more modern network have more expressive feature extractors and
            % thus activations that can be linearly classified. 
            % Consequently, utilising a CVAE with significantly lower expressive power to estimate
            % the activations of networks such as AlexNet and VGG where activations cannot be
            % linearly classified, is challenging. 
            Consequently, utilising a CVAE, with significantly lower expressive power than a
            feature extractor, to estimate the activations of networks such as AlexNet and VGG is
            challenging. 
            Furthermore, the dimensionality of the input to VGG11's feature extractor has 10,388
            neurons making it challenging to create a CVAE architecture with a reasonable memory
            footprint to estimate so many neurons.  
            Preliminary results fail to successfully train small VAEs to estimate the activations
            of VGG11 and further exploration of this limitation is left for future work.
    
    \subsection{Unconditional vs Conditional VAEs}
        \label{sec:fe_uncon_con}
        \input{tables_tex/further_experiments/uncon_con.tex}
        Instead of training a single CVAE for all 1000 classes of ILSVRC'12, it is possible to
        train smaller unconditional VAEs per class and depending on the activation desired, the
        appropriate VAE is sampled.  
        The architecture of the VAE used is provided in Appendix \ref{app:vae_archs}, and each VAE
        consumes only 0.4 MB. 
        This experiment explores if conditioning the VAE on classes causes any loss in
        representation capabilities.
        Table.\ref{tab:uncon_con_comparison} shows the results for no label space uncertainty
        retraining of $\mathcal{M}^{80}_{TFO}$ for various $\mathcal{D}'$ using LoCO-PDA.
        The results demonstrate that on average across $\mathcal{D}'$, the unconditional approach
        performs 0.22pp worse than one CVAE while consuming 40x more memory.
        Thus, a conditional architecture has significant memory benefits and similar representation
        capabilities as the unconditional architecture. 



==> figs_tex/background/vae_training.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[trim={0 1cm 0 0},clip,width=0.5\textwidth]{figs/background/vae_diagram.png}
    \caption{Conditional VAE Training (Left) and Inference (Top Right) Processes \cite{2021_vae_tutorial}}
    \label{fig:vae_training}
    % \vspace{-0.5cm}
\end{figure}


==> figs_tex/methodology/network_change.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=0.5\textwidth]{figs/methodology/network_change.pdf}
    % \includegraphics[trim={5.7cm 12.5cm 11.7cm 4.5cm},clip,width=0.4\textwidth]{figs/methodology/proposed_methodology.pdf}
    \includegraphics[trim={5.7cm 12.8cm 9.8cm 3.9cm},clip,width=0.5\textwidth]{figs/methodology/proposed_method.pdf}
    \caption{Visualisation of the proposed retraining strategy}
    \label{fig:retraining_strategy}
    \vspace{-0.5cm}
\end{figure}


==> tables_tex/evaluation/training_approaches_mem_footprint_comparison.tex <==
\begin{table}[t]
    \begin{minipage}[b]{\linewidth}
    \begin{small}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{lcccc}
            \toprule
            & \textbf{\textsc{City}} & \textbf{\textsc{Motorway}} & \textbf{\textsc{Country-side}} & \textbf{\textsc{Off-road}} \\
            \midrule
            \textbf{\textsc{Memory (GB)}} & 9.40 & 1.36 & 10.3 & 1.36 \\
            \bottomrule
        \end{tabular}
    }
    \end{small}
    \caption{Memory footprint of storing all images in the retraining dataset for each $\mathcal{D}'$}
    \label{tab:unlim_mem_footprint}
    % \vspace{-0.5cm}
    \end{minipage}
\end{table}


==> tables_tex/evaluation/vae_acc_comparison.tex <==
\begin{table}[t]
    \begin{minipage}[b]{\linewidth}
    \begin{small}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|c|c|c|c|c}
            \toprule
            & \multicolumn{2}{c|}{\textbf{\textsc{All Layers}}} & \multicolumn{3}{c}{\textbf{\textsc{Classifier Only}}} \\
            \cmidrule(lr){2-6}
            & \textsc{TFO} & \textsc{OFA} & \textsc{TFO} & \textsc{OFA} & \textsc{PersEPhonEE} \\
            \midrule
            \textbf{\textsc{Memory Limited}} & 76.88 & 81.44 & 75.15 & 81.44 & 23.79 \\
            \textbf{\textsc{Memory Unlimited}} & 81.19 & 79.59 & 79.22 & 84.63 & 26.70 \\
            \bottomrule
        \end{tabular}
    }
    \end{small}
    \caption{Best achieved Top1-Test accuracy for the various baseline approaches to on-device retraining. Values are averaged over all four autonomous driving $\mathcal{D}'$.}
    \label{tab:baseline_acc}
    \vspace{-0.5cm}
    \end{minipage}
\end{table}


==> tables_tex/further_experiments/mobilenet_v2_80_acc.tex <==
\begin{table}[t]
    \begin{minipage}[b]{\linewidth}
    \begin{small}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{lc ccc cc}
            \toprule
            & & \multicolumn{5}{c}{\textsc{$\mathcal{M}^{80}_{TFO}$ (\%)}} \\ 
            \cmidrule(lr){3-7}
            & \textsc{$\mathcal{M}^{0}_{TFO}$ (\%)}& \multicolumn{3}{c}{\textsc{No Uncertainty}} & \multicolumn{2}{c}{\textsc{Uncertainty}} \\ 
            \cmidrule(lr){3-5}
            \cmidrule(lr){6-7}
            & \textsc{No Retrain} & \textsc{No Retrain} & \textsc{Retrained} & \textbf{\textsc{VAE}} & \textsc{Retrained} & \textbf{\textsc{VAE}} \\
            \midrule
            \textbf{\textsc{City} (185)}           & 74.44  & 50.11 & 53.91 & 52.13 &  &  \\
            \textbf{\textsc{Motorway} (26)}        & 72.03  & 50.08 & 63.13 & 62.76 &  &  \\
            \textbf{\textsc{Country-side} (204)}   & 74.96  &  & & 53.29 &  &  \\
            \textbf{\textsc{Off-road} (26)}        & 78.85  & 54.02 & 76.91 & 76.40 &  &  \\
            \bottomrule
        \end{tabular}
    }
    \end{small}
    \caption{Pre and post on-device domain adaptation accuracy of a 50\% pruned MobileNetV2 network. 
             The table titles are the same as in Table.\ref{tab:acc_comparison}.}
    \label{tab:mobv2_acc_comparison}
    \vspace{-0.5cm}
    \end{minipage}
\end{table}

